LACIN: Linearly Arranged Complete Interconnection Networks

Several interconnection networks are based on the complete graph topology. Networks with a moderate size can be based on a single complete graph. However, large-scale networks such as Dragonfly and HyperX use, respectively, a hierarchical or a multi-dimensional composition of complete graphs. The number of links in these networks is huge and grows rapidly with their size. This paper introduces LACIN, a set of complete graph implementations that use identically indexed ports to link switches. This way of implementing the network reduces the complexity of its cabling and its routing. LACIN eases the deployment of networks for parallel computers of different scales, from VLSI systems to the largest supercomputers.

==> code.tex <==

\usepackage{tikz}
\usepackage{ifthen}
\usetikzlibrary{decorations.pathreplacing}%brace decoration


\makeatletter
\xdef\lacin@lane{0}%A default to avoid undefined use.
\xdef\columnhighlight{9999}
\tikzset{
	wire/.style={thick},
	%wire/.style={thick,every edge/.style={looseness=1}},
}

\pgfmathdeclarefunction{xor}{2}{%
	% divide(x,y),iseven(x),greater(x,y)
	\pgfmathtruncatemacro\first{#1}%
	\pgfmathtruncatemacro\second{#2}%
	\def\accumulator{0}%
	\def\value{1}%
	%\typeout{first=\first, second=\second}%
	%\typein{}%
	\whiledo{\second>0}{%
		\pgfmathparse{1-equal( mod(\first,2), mod(\second,2) )}%
		\pgfmathtruncatemacro\accumulator{\accumulator + \pgfmathresult*\value}%
		\pgfmathtruncatemacro\value{2*\value}%
		\pgfmathtruncatemacro\first{divide(\first,2)}%
		\pgfmathtruncatemacro\second{divide(\second,2)}%
		%\typeout{first=\first, second=\second}
		%\typein{}
	}%
	\pgfmathparse{\first*\value+\accumulator}%
}

%%% Count Trailing Zeros
\pgfmathdeclarefunction{CTZ}{1}{%
	\pgfmathtruncatemacro\argument{#1}%
	\def\accumulator{0}%
	\pgfmathparse{iseven(\argument)}%
	\whiledo{\pgfmathresult=1}{%
		\pgfmathtruncatemacro\argument{divide(\argument,2)}%
		\pgfmathtruncatemacro\accumulator{\accumulator + 1}%
		\pgfmathparse{iseven(\argument)}%
	}%
	\pgfmathparse{\accumulator}%
}

%%% 2 to the power of CTZ(n)
\pgfmathdeclarefunction{powCTZ}{1}{%
	\pgfmathtruncatemacro\argument{#1}%
	\def\accumulator{1}%
	\pgfmathparse{iseven(\argument)}%
	\whiledo{\pgfmathresult=1}{%
		\pgfmathtruncatemacro\argument{divide(\argument,2)}%
		\pgfmathtruncatemacro\accumulator{\accumulator * 2}%
		\pgfmathparse{iseven(\argument)}%
	}%
	\pgfmathparse{\accumulator}%
}


\pgfmathdeclarefunction{cayley}{3}{%
	\pgfmathtruncatemacro\origin{#1}%
	\pgfmathtruncatemacro\port{#2}%
	\pgfmathtruncatemacro\size{#3}%
	\pgfmathtruncatemacro\exponente{floor(log2(2.01+\port))}%
	\pgfmathtruncatemacro\M{pow(2,\exponente)}%
	\pgfmathparse{xor(\origin,1+\port)}%
	\xdef\lacin@target{\pgfmathresult}%
	\pgfmathtruncatemacro\excess{mod(\lacin@target,\M)}%
	\xdef\lacin@lane{\excess}%
	\xdef\lacin@numlanes{\M}%
	\pgfmathparse{\lacin@target}%
}

\pgfmathdeclarefunction{enrique}{3}{%
	\pgfmathtruncatemacro\origin{#1}% from 0 to size-1
	\pgfmathtruncatemacro\port{#2}% from 0 to size-2
	\pgfmathtruncatemacro\enrique@size{#3}%
	\pgfmathtruncatemacro\enrique@evensize{\enrique@size + isodd(\enrique@size)}%
	%INVARIANT evensize = 2^u * v
	\pgfmathtruncatemacro\v{\enrique@evensize}%
	\pgfmathtruncatemacro\u{0}%
	\pgfmathtruncatemacro\powu{1}%
	\pgfmathparse{iseven(\v)}%
	\whiledo{\pgfmathresult=1}{%
		\pgfmathtruncatemacro\v{divide(\v,2)}%
		\pgfmathtruncatemacro\u{\u + 1}%
		\pgfmathtruncatemacro\powu{2*\powu}%
		\pgfmathparse{iseven(\v)}%
	}%
	%  evensize = 2^u * v, with v odd
	\pgfmathtruncatemacro\k{\port}%
	%\typeout{v=\v, powu=\powu, k=\k, s=\s, sv=\sv, sacc=\sacc}%
	%\pgfmathtruncatemacro\lacin@lane{random(0,9)}%
	%\pgfmathtruncatemacro\lacin@numlanes{10}%
	\pgfmathtruncatemacro\lacin@numlanes{\enrique@evensize/2}%
	\pgfmathtruncatemacro\lacin@lane{Mod(\origin,\lacin@numlanes)}%
	\xdef\lacin@lane{\lacin@lane}%
	\xdef\lacin@numlanes{\lacin@numlanes}%
	\pgfmathtruncatemacro\case{\k+\v+1<\enrique@evensize}%
	%\ifthenelse{\sacc<\enrique@evensize}{%
	%\ifthenelse{\s<\u}{%
	\ifthenelse{\case=1}{%
		\pgfmathtruncatemacro\s{1}%
		\pgfmathtruncatemacro\sv{\powu/2*\v}%
		\pgfmathtruncatemacro\sacc{\sv}%
		\pgfmathtruncatemacro\cond{\k>=\sacc}%
		%\whiledo{\k>\sacc}{%
		\whiledo{\cond=1}{%
			\pgfmathtruncatemacro\s{\s + 1}%
			\pgfmathtruncatemacro\sv{divide(\sv,2)}%
			\pgfmathtruncatemacro\sacc{\sacc+\sv}%
			\pgfmathtruncatemacro\cond{\k>=\sacc}%
		}%
		%Found the first \s such that the sum of  v*2^(u-i) with i from 1 to s is greater than the port index k.
		\pgfmathtruncatemacro\pows{pow(2,\s-1)}%
		\pgfmathtruncatemacro\q{divide(\origin,\pows)}%
		\pgfmathtruncatemacro\d{ \k + \sv - \sacc }%
		\pgfmathtruncatemacro\eps{iseven(\d)}% in {0,1}
		\pgfmathtruncatemacro\d{ \d+\eps }%
		% \d is guaranteed to be odd.  k= d +eps +sum
		\pgfmathtruncatemacro\lacin@numlanes{\k+1}%
		%\pgfmathtruncatemacro\lacin@numlanes{\d+1}%
		%\xdef\lacin@numlanes{\lacin@numlanes}%
		%\pgfmathtruncatemacro\lacin@lane{Mod(\origin,\lacin@numlanes)}%
		%\xdef\lacin@lane{\lacin@lane}%
		%\typeout{origin=\origin, pows=\pows, s=\s}%
		\pgfmathtruncatemacro\dir{pow(-1, \q+\eps+1)}%
		\pgfmathtruncatemacro\lacin@lane{divide(\q,2)+Mod(\origin,\pows)}%
		\pgfmathtruncatemacro\lacin@lane{\lacin@lane+(\dir-1)*\lacin@numlanes/4}%
		\xdef\lacin@lane{\lacin@lane}%
		\xdef\lacin@numlanes{\lacin@numlanes}%
		%\pgfmathtruncatemacro\lacin@lane{mod(\d,\pows)}%
		%\pgfmathtruncatemacro\lacin@numlanes{\sacc}%
		%\xdef\lacin@lane{0}%
		%\xdef\lacin@numlanes{1}%
		\pgfmathparse{Mod(\origin + \pows*\dir*\d,\enrique@evensize)}%
		\xdef\lacin@target{\pgfmathresult}%
	}{%
		%\pgfmathtruncatemacro\current{\enrique@evensize}%
		%\pgfmathtruncatemacro\uacc{0}%
		%\pgfmathtruncatemacro\final{\u-1}%
		%\foreach \i in {1,...,\final}{%
		%	\pgfmathtruncatemacro\current{\current /2}%
		%	\pgfmathtruncatemacro\uacc{\uacc+\current}%
		%	\xdef\current{\current}%
		%	\xdef\uacc{\uacc}%
		%}%
		%\pgfmathtruncatemacro\t{ \k+1 - \uacc }%
		\pgfmathtruncatemacro\t{ \k+\v+1-\enrique@evensize }%
		\pgfmathtruncatemacro\q{divide(\origin,\powu/2)}%
		\pgfmathtruncatemacro\r{Mod(\origin,\powu/2)}%
		%\pgfmathtruncatemacro\cond{(Mod(\q,\v)-\t)==0}%
		\pgfmathtruncatemacro\cond{(\q==\t) || (\q==\t+\v)}%
		%\typeout{k=\k, cond=\cond, q=\q, t=\t, powu=\powu, size=\enrique@evensize, uacc=\uacc, u=\u}%
		\pgfmathtruncatemacro\factor{ (\q+\v)*\cond + (2*\t-\q)*(1-\cond) }%
		\pgfmathparse{Mod(\r+\powu/2*\factor,\enrique@evensize)}%
		%\pgfmathparse{\cond}%
		\xdef\lacin@target{\pgfmathresult}%
	}%
	%\typeout{origin=\origin, target=\lacin@target, q=\q, eps=\eps, dir=\dir, pows=\pows, d=\d}%
}
\pgfmathdeclarefunction{enrique2}{3}{%
	\pgfmathtruncatemacro\origin{#1}% from 0 to size-1
	\pgfmathtruncatemacro\port{#2}% from 0 to size-2
	\pgfmathtruncatemacro\enrique@size{#3}%
	\pgfmathtruncatemacro\minoffset{powCTZ(\enrique@size)}%
	\pgfmathtruncatemacro\halfsize{\enrique@size / 2}%
	\pgfmathtruncatemacro\halfport{\port / 2}%
	\pgfmathtruncatemacro\basedirection{Mod(\port,2)}%
	%% Get the offset.
	%% Offsets increase sequentially per halfport, starting at 1 with limit offset<n/2,
	%% and skipping those multiples of minoffset.
	%% Thus, offset is about (minoffset+1)/minoffset * halfport
	%% offset = 1 + halfport + quo(halfport,minoffset)
	\pgfmathtruncatemacro\skipped{(1+\halfport)/\minoffset}%
	\pgfmathtruncatemacro\offset{1 + \halfport + \skipped}%
	\pgfmathtruncatemacro\blocksize{ powCTZ(\offset) }%
	\pgfmathtruncatemacro\block{\origin / \blocksize}%
	\pgfmathtruncatemacro\direction{Mod(\basedirection + \block,2)}%
	\ifthenelse{\offset<\halfsize}{%
		\pgfmathparse{Mod(\origin+\offset*pow(-1,\direction),\enrique@size)}%
		\xdef\lacin@target{\pgfmathresult}%
	}{%
		%% Then the offset must change depending on the block.
		%% First block at the first of these ports to use offset=+maxoffset
		%% Each block then having the offset reduced by minoffset
		%% Until 0, which is replaced by n/2.
		%% But we continue subtracting as it were 0, until reaching -maxoffset.
		%% Further ports are shifts, equivalently as subtracting one block.
		%% There are n/\minoffset of these ports, so the first one is at n-1-n/\minoffset.
		\pgfmathtruncatemacro\maxoffset{\halfsize-\minoffset/2}%
		\pgfmathtruncatemacro\block{\origin / (\minoffset/2)}%
		\pgfmathtruncatemacro\portoffset{\port - (\enrique@size-1-\enrique@size/\minoffset) }%
		\pgfmathtruncatemacro\offset{ Mod( \maxoffset - \minoffset*(\block-\portoffset), \enrique@size )}%
		\pgfmathtruncatemacro\offset{ \offset + equal(\offset,0)*\halfsize }%
		\pgfmathparse{Mod(\origin+\offset,\enrique@size)}%
		\xdef\lacin@target{\pgfmathresult}%
	}%
	\xdef\lacin@lane{0}%
	\xdef\lacin@numlanes{1}%
}

\pgfmathdeclarefunction{circle}{3}{%
	\pgfmathtruncatemacro\origin{#1}% from 0 to size-1
	\pgfmathtruncatemacro\circle@port{#2}% from 0 to size-2
	\pgfmathtruncatemacro\circle@size{#3+isodd(#3)}%next even
	%\pgfmathtruncatemacro\circle@port{Mod(\circle@port+1,\circle@size-1)}%shift to make port 1 of center go to switch 1.
	\ifthenelse{\origin=\circle@size-1}{%
		%%Connect the center
		\xdef\lacin@target{\circle@port}%
	}{%
		\ifthenelse{\origin=\circle@port}{%
			%%Connect the center pair
			\pgfmathparse{\circle@size-1}%
			\xdef\lacin@target{\pgfmathresult}%
		}{%
			\pgfmathparse{Mod(2*\circle@port-\origin,\circle@size-1)}%
			\xdef\lacin@target{\pgfmathresult}%
		}%
	}%
	\xdef\lacin@lane{0}%
	\xdef\lacin@numlanes{1}%
}

% For dash patterns see from page 168 in the pgf manual.
\expandafter\def\csname lacin@dashpattern@0\endcsname{solid}%
\expandafter\def\csname lacin@dashpattern@1\endcsname{densely dashed}%
\expandafter\def\csname lacin@dashpattern@2\endcsname{densely dotted}%
\expandafter\def\csname lacin@dashpattern@3\endcsname{densely dash dot}%
\expandafter\def\csname lacin@dashpattern@4\endcsname{densely dash dot dot}%
\expandafter\def\csname lacin@dashpattern@5\endcsname{dashed}%
\expandafter\def\csname lacin@dashpattern@6\endcsname{dotted}%
\expandafter\def\csname lacin@dashpattern@7\endcsname{dash dot}%
\expandafter\def\csname lacin@dashpattern@8\endcsname{dash dot dot}%
\expandafter\def\csname lacin@dashpattern@9\endcsname{loosely dashed}%
\expandafter\def\csname lacin@dashpattern@10\endcsname{loosely dotted}%
\expandafter\def\csname lacin@dashpattern@11\endcsname{loosely dash dot}%
\expandafter\def\csname lacin@dashpattern@12\endcsname{loosely dash dot dot}%
\def\lacin@numdashpatterns{1}
\newcommand{\lanestyle}{%
	%\pgfmathsetmacro\red{100*\lacin@lane/\lacin@numlanes}%
	%\tikzset{lane/.style={draw=red!\red!blue,thick}}%
	\pgfmathtruncatemacro\pat{Mod(\lacin@lane,\lacin@numdashpatterns)}%
	\edef\tmpdashpattern{\csname lacin@dashpattern@\pat\endcsname}
	\tikzset{lane/.style={\tmpdashpattern}}%
}

\newcommand{\portcolumn}[3]{%
%\typeout{portcolumn: 1=#1 2=#2}
%\typein{}
\def\portcolumn@size{#1}
\def\portcolumn@port{#2}
\def\portcolumn@function{#3}
%\pgfmathtruncatemacro\exponente{floor(log2(1.01+\port))}
%\pgfmathtruncatemacro\M{pow(2,\exponente)}
%\typeout{portcolumn: size=\portcolumn@size port=\portcolumn@port}
%\typein{}
\foreach \nextindex in {1,...,\portcolumn@size}
{
	\pgfmathtruncatemacro{\index}{\nextindex-1}
	%\path[draw] (0,-\index) circle (3pt) node [anchor=east] {\index};
	\path[draw] (0,-\index) circle (3pt);
	\pgfmathtruncatemacro{\destination}{\portcolumn@function(\index,\portcolumn@port,\portcolumn@size)}%
	\pgfmathtruncatemacro{\cond}{\destination>\index && \destination<\portcolumn@size}
	\ifthenelse{\cond=1}{
		%%\pgfmathsetmacro\dist{abs(\destination - \index)}
		%\pgfmathsetmacro\excess{mod(\destination,\M)}
		%%\pgfmathsetmacro\red{100*\index/\portcolumn@size}
		%%\pgfmathsetmacro\blue{100*mod(\index,4)/4}
		%\pgfmathsetmacro\red{100*\excess/\M}
		%%\pgfmathsetmacro\blue{100*mod(\index,4)/4}
		%%\draw[->,draw=red!\red!blue!\blue!gray]
		%\draw[->,draw=red!\red!blue,thick]
		%	(0,-\index) -- ++(5pt + 3pt*\excess,0) |- (0,-\destination);
		%\typeout{lane=\lacin@lane numlanes=\lacin@numlanes target=\lacin@target}
		%\draw[->,draw=red!\red!blue,thick]
		\lanestyle
		%\draw[lane,thick] (0,-\index) -- ++(5pt + 3.0pt*\lacin@lane,0) |- (0,-\lacin@target);
		%
		%%downwards
		%\draw[lane,thick] (0,-\index) edge [out=-70,in=70] (0,-\lacin@target);
		%%upwards
		\draw[lane,wire,overlay] (0,-\portcolumn@size+1+\index) edge [out=70,in=-70] (0,-\portcolumn@size+1+\lacin@target);
	}{}
}
}


\newcommand{\complete}[2]{%
\def\complete@size{#1}%
\def\complete@function{#2}%
\pgfmathtruncatemacro\lastport{\complete@size - 2 + isodd(\complete@size)}%
\pgfmathtruncatemacro\lastindex{\complete@size - 1}%
\foreach \port in {0,...,\lastport}
{
	%\pgfmathsetmacro\extra{floor(log2(1.01+\port))}
	\def\extra{0}
	\begin{scope}[xshift=\port*40pt + \extra*20pt]
	\ifthenelse{\port=\columnhighlight}{\tikzset{
		wire/.style={ultra thick}
		%wire/.style={ultra thick,every edge/.append style={looseness=1.5}}
	}}{}
	\portcolumn{\complete@size}{\port}{\complete@function}
	\end{scope}
}
\foreach \index in {0,...,\lastindex}
{
	%%downwards
	%\path[draw] (0,-\index) node [anchor=east,shift={(-10pt,0)}] (label\index) {Switch \index};
	%%upwards
	\path[draw] (0,-\lastindex+\index) node [anchor=east,shift={(-10pt,0)}, font=\scriptsize] (label\index) {$S= \index$};
	\draw[thin] (0,-\index) ++(-10pt,-5pt) rectangle ++(\lastport*40pt+40pt,.5);
}
}


%% Complete extended with server ports.
\newcommand{\completeextended}[2]{%
\def\complete@size{#1}%
\def\complete@function{#2}%
\pgfmathtruncatemacro\lastport{\complete@size - 2 + isodd(\complete@size)}%
\pgfmathtruncatemacro\lastindex{\complete@size - 1}%
\foreach \port in {0,...,\lastport}
{
	\begin{scope}[xshift=\lastport*40pt - \port*40pt]
	\portcolumn{\complete@size}{\port}{\complete@function}
	\end{scope}
}
\foreach \port in {1,...,\complete@size}
{
	\begin{scope}[xshift=\complete@size*40pt - \port*40pt + \lastport*40pt + 40pt]
	\foreach \index in {0,...,\lastindex}
	{
		\path[draw] (0,-\index) circle (3pt);
	}
	\end{scope}
}
\foreach \index in {0,...,\lastindex}
{
	%%downwards
	%\path[draw] (0,-\index) node [anchor=east,shift={(-10pt,0)}] (label\index) {Switch \index};
	%%upwards
	\path[draw] (0,-\lastindex+\index) node [anchor=east,shift={(-10pt,0)}] (label\index) {$S= \index$};
	\draw[thin] (0,-\index) ++(-10pt,-5pt) rectangle ++(2*\lastport*40pt+120pt,.5);
}
}

%% Complete extended with server ports.
\newcommand{\completeextelipsis}[2]{%
\def\complete@size{#1}%
\def\complete@function{#2}%
\pgfmathtruncatemacro\lastport{\complete@size - 2 + isodd(\complete@size)}%
\pgfmathtruncatemacro\lastindex{\complete@size - 1}%
\foreach \port in {0,...,\lastport}
{
	%\begin{scope}[xshift=\lastport*40pt - \port*40pt]
	\begin{scope}[xshift=\port*40pt]
	\portcolumn{\complete@size}{\port}{\complete@function}
	\end{scope}
}
\foreach \port in {1,3}
{
	%\begin{scope}[xshift=160pt - \port*40pt + \lastport*40pt]
	\begin{scope}[xshift=\lastport*40pt + \port*40pt]
	\foreach \index in {0,...,\lastindex}
	{
		\path[draw] (0,-\index) circle (3pt);
	}
	\end{scope}
}
%\begin{scope}[xshift=80pt + \lastport*40pt]
\begin{scope}[xshift=\lastport*40pt + 80pt]
\foreach \index in {0,...,\lastindex}
{
	\path[draw] (0,-\index) node {\ldots};
}
\end{scope}
\foreach \index in {0,...,\lastindex}
{
	%%downwards
	%\path[draw] (0,-\index) node [anchor=east,shift={(-10pt,0)}] (label\index) {Switch \index};
	%%upwards
	\path[draw] (0,-\lastindex+\index) node [anchor=east,shift={(-10pt,0)}] (label\index) {Switch \index};
	\draw[thin] (0,-\index) ++(-10pt,-5pt) rectangle ++(\lastport*40pt+160pt,.5);
}
}

\newcommand{\targettable}[2]{%
\typeout{Enter targettable 1=#1 2=#2}%
\def\complete@size{#1}%
\def\complete@function{#2}%
\pgfmathtruncatemacro\lastsize{\complete@size - 1}%
\pgfmathtruncatemacro\lastport{\complete@size - 2 + isodd(\complete@size)}%
%\typeout{loop outisde tikz}%
\xdef\tableheader{}%
\foreach \port in {0,...,\lastport}{%
	\xdef\tableheader{\tableheader |c}%
}%
\xdef\firstline{}%
\foreach \port in {0,...,\lastport}{%
	\xdef\firstline{\firstline &\port}%
}%
\xdef\rows{}%
\typeout{Enter targettable main loop}%
\foreach \rowindex in {0,...,\lastsize}{%
	\xdef\row{\rowindex}%
	\foreach \port in {0,...,\lastport}{%
		%\pgfmathtruncatemacro\inc{\complete@function(\rowindex,\port,\complete@size) - \rowindex}
		\pgfmathtruncatemacro\destination{\complete@function(\rowindex,\port,\complete@size)}%
		\ifthenelse{\destination<\complete@size}{%
			\pgfmathtruncatemacro\inc{\destination - \rowindex}%
		}{
			\def\inc{-}%
		}%
		\xdef\row{\row &\inc}%
	}%
	\xdef\rows{\rows \row\\}%
}%
\typeout{Finished targettable main loop. Got tableheader=\tableheader}%
%\typein{}
\edef\tmp{{tabular}{|c|\tableheader|}}%
\setlength{\tabcolsep}{1pt}%default 6pt?
%\begin{tabular}{|c|\tableheader|}
\expandafter\begin\tmp
\hline
\firstline\\
\hline
\rows
\hline
\end{tabular}
\typeout{Finished targettable}
}

\newcommand{\hamming}[4]{%
\def\hamming@horizontal@size{#1}%
\def\hamming@horizontal@function{#2}%
\def\hamming@vertical@size{#3}%
\def\hamming@vertical@function{#4}%
%\pgfmathsetlength{\routersize}{.8}%
\pgfmathsetmacro{\routersize}{.8}%
\pgfmathsetmacro{\portlineoffset}{.08}%
\pgfmathsetmacro{\firstportoffset}{.2}%
\pgfmathsetmacro{\horizontalportsize}{(\routersize-\firstportoffset)/(\hamming@vertical@size-1+isodd(\hamming@vertical@size))}%
\pgfmathsetmacro{\verticalportsize}{(\routersize-\firstportoffset)/(\hamming@horizontal@size-1+isodd(\hamming@horizontal@size))}%
\pgfmathtruncatemacro\lasthorizontal{\hamming@horizontal@size - 1}%
\pgfmathtruncatemacro\lastvertical{\hamming@vertical@size - 1}%
\tikzset{port/.style={circle,draw,inner sep=0,minimum width=3pt}}
\foreach \horizontalindex in {0,...,\lasthorizontal}
{
	\foreach \verticalindex in {0,...,\lastvertical}
	{
		%\draw (\horizontalindex,\verticalindex) ++(-.4,-.4) rectangle ++(.8,.8);
		\draw (\horizontalindex,\verticalindex) rectangle ++(\routersize,\routersize);
	}
}
\foreach \horizontalindex in {0,...,\lasthorizontal}
{
	%\pgfmathsetmacro\extra{floor(log2(1.01+\port))}
	%\def\extra{0}
	%\begin{scope}[xshift=\port*40pt + \extra*20pt]
	%\portcolumn{\complete@size}{\port}{\complete@function}
	%\end{scope}
	\foreach \verticalindex in {0,...,\lastvertical}
	{
		%horizontal lines
		\pgfmathtruncatemacro\lastport{\hamming@horizontal@size - 2 + isodd(\hamming@horizontal@size)}%
		\foreach \portindex in {0,...,\lastport}
		{
			\path  (\horizontalindex,\verticalindex) ++(\portlineoffset,\firstportoffset+\verticalportsize*\portindex) node[port] {};
			\pgfmathtruncatemacro{\destination}{\hamming@horizontal@function(\horizontalindex,\portindex,\hamming@horizontal@size)}%
			\pgfmathtruncatemacro{\cond}{\destination>\horizontalindex && \destination<\hamming@horizontal@size}
			\ifthenelse{\cond=1}{
				\lanestyle
				%\draw[lane,thick] (\horizontalindex,\verticalindex) ++(\portlineoffset,0) -- ++(2pt+1pt*\portindex,1pt + 2.0pt*\lacin@lane + 1pt*\portindex) -| (\lacin@target,\verticalindex);
				\path (\horizontalindex,\verticalindex) ++(\portlineoffset,\firstportoffset+\verticalportsize*\portindex) coordinate (s) ++(0,2pt + 2.0pt*\lacin@lane ) coordinate(sm);
				\path (\lacin@target,\verticalindex) ++(\portlineoffset,\firstportoffset+\verticalportsize*\portindex) coordinate (e) ++(0,2pt + 2.0pt*\lacin@lane ) coordinate(em);
				%\draw[lane,thick] (s) -- (sm) -- (em) -- (e);
				\draw[lane,thick] (s) edge[out=10,in=170] (e);
			}{}
		}
		%vertical lines
		\pgfmathtruncatemacro\lastport{\hamming@vertical@size - 2 + isodd(\hamming@vertical@size)}%
		\foreach \portindex in {0,...,\lastport}
		{
			\path  (\horizontalindex,\verticalindex) ++(\firstportoffset+\horizontalportsize*\portindex,\portlineoffset) node[port] {};
			\pgfmathtruncatemacro{\destination}{\hamming@vertical@function(\verticalindex,\portindex,\hamming@vertical@size)}%
			\pgfmathtruncatemacro{\cond}{\destination>\verticalindex && \destination<\hamming@vertical@size}
			\ifthenelse{\cond=1}{
				\lanestyle
				%\draw[lane,thick] (\horizontalindex,\verticalindex) ++(0,\portlineoffset) -- ++(1pt + 2.0pt*\lacin@lane + 1pt*\portindex,2pt+1pt*\portindex) |- (\horizontalindex,\lacin@target);
				\path (\horizontalindex,\verticalindex) ++(\firstportoffset+\horizontalportsize*\portindex,\portlineoffset) coordinate (s) ++(2pt + 2.0pt*\lacin@lane ,0) coordinate (sm);
				\path (\horizontalindex,\lacin@target) ++(\firstportoffset+\horizontalportsize*\portindex,\portlineoffset) coordinate (e) ++(2pt + 2.0pt*\lacin@lane ,0) coordinate (em);
				%\draw[lane,thick] (s) -- (sm) -- (em) -- (e);
				\draw[lane,thick] (s) edge[out=80,in=-80] (e);
			}{}
		}
	}
}
%\foreach \index in {0,...,\lastindex}
%{
%	\path[draw] (0,-\index) node [anchor=east,shift={(-10pt,0)}] {\index};
%	\draw[very thick] (0,-\index) ++(-10pt,-5pt) rectangle ++(\lastport*40pt+40pt,.5);
%}
}

\newcommand{\bicomplete}[4]{%
\def\hamming@horizontal@size{#1}%
\def\hamming@horizontal@function{#2}%
\def\hamming@vertical@size{#3}%
\def\hamming@vertical@function{#4}%
\pgfmathtruncatemacro\lasthorizontal{\hamming@horizontal@size - 1}%
\pgfmathtruncatemacro\lastvertical{\hamming@vertical@size - 1}%
\foreach \horizontalindex in {0,...,\lasthorizontal}
{
	\foreach \verticalindex in {0,...,\lastvertical}
	{
		\expandafter\xdef\csname horizontalreverse\horizontalindex to\verticalindex\endcsname{-1}
		\expandafter\xdef\csname verticalreverse\horizontalindex to\verticalindex\endcsname{-1}
		\draw (\horizontalindex,\verticalindex) ++(-.4,-.4) rectangle ++(.8,.8);
	}
}
\typeout{build reverse horizontal function}
\foreach \horizontalindex in {0,...,\lasthorizontal}
{
	%\expandafter\xdef\csname horizontalreverse\horizontalindex to\horizontalindex\endcsname{-1}
	\pgfmathtruncatemacro\lastport{\hamming@horizontal@size - 2}%
	\foreach \portindex in {0,...,\lastport}
	{
		\pgfmathtruncatemacro{\destination}{\hamming@horizontal@function(\horizontalindex,\portindex,\hamming@horizontal@size)}%
		\expandafter\xdef\csname horizontalreverse\horizontalindex to\destination\endcsname{\portindex}
	}
}
\typeout{build reverse vertical function}
\foreach \verticalindex in {0,...,\lastvertical}
{
	%\expandafter\xdef\csname verticalreverse\verticalindex to\verticalindex\endcsname{-1}
	\pgfmathtruncatemacro\lastport{\hamming@vertical@size - 2}%
	\foreach \portindex in {0,...,\lastport}
	{
		\pgfmathtruncatemacro{\destination}{\hamming@vertical@function(\verticalindex,\portindex,\hamming@vertical@size)}%
		\expandafter\xdef\csname verticalreverse\verticalindex to\destination\endcsname{\portindex}
	}
}
\typeout{drawing lines}
\foreach \horizontalindex in {0,...,\lasthorizontal}
{
	%\pgfmathsetmacro\extra{floor(log2(1.01+\port))}
	%\def\extra{0}
	%\begin{scope}[xshift=\port*40pt + \extra*20pt]
	%\portcolumn{\complete@size}{\port}{\complete@function}
	%\end{scope}
	\foreach \verticalindex in {0,...,\lastvertical}
	{
		\pgfmathtruncatemacro\fullindex{\horizontalindex + \verticalindex*\hamming@horizontal@size}
		\foreach \targethorizontalindex in {0,...,\lasthorizontal}
		{
			\foreach \targetverticalindex in {0,...,\lastvertical}
			{
				\pgfmathtruncatemacro\targetfullindex{\targethorizontalindex + \targetverticalindex*\hamming@horizontal@size}
				\ifthenelse{\fullindex=\targetfullindex}{}{
					\path (\horizontalindex,\verticalindex) ++(-15pt+17pt*\targethorizontalindex,-15pt+17pt*\targetverticalindex) coordinate (s);
					\path (\targethorizontalindex,\targetverticalindex) ++(-15pt+17pt*\horizontalindex,-15pt+17pt*\verticalindex) coordinate (e);
					\draw (s) circle(2pt);
				}
				\ifthenelse{\fullindex<\targetfullindex}{
					\edef\horizontalport{\csname horizontalreverse\horizontalindex to\targethorizontalindex\endcsname}
					\edef\verticalport{\csname verticalreverse\verticalindex to\targetverticalindex\endcsname}
					\pgfmathtruncatemacro\lacin@lane{Mod(\lacin@lane+1,\lacin@numlanes)}
					\xdef\lacin@lane{\lacin@lane}
					\lanestyle
					\ifthenelse{\horizontalport=-1}{
							%pure vertical
							\path (s) ++(1pt+3pt*\verticalport,0) coordinate (sm);
							\path (e) ++(1pt+3pt*\verticalport,0) coordinate (em);
							\draw[lane,thick] (s) -- (sm) -- (em) -- (e);
					}{
						\ifthenelse{\verticalport=-1}{
							%pure horizontal
							\path (s) ++(0,1pt+3pt*\horizontalport) coordinate (sm);
							\path (e) ++(0,1pt+3pt*\horizontalport) coordinate (em);
							\draw[lane,thick] (s) -- (sm) -- (em) -- (e);
						}{
							%DOR lines
							%\draw (\horizontalindex,\verticalindex) -- (\targethorizontalindex,\targetverticalindex);
							%\path (\horizontalindex,\verticalindex) ++(-10pt+17pt*\targethorizontalindex,-45pt+10pt*\horizontalport+2pt*\verticalport) coordinate (sm);
							\path (s) ++(1pt+3pt*\verticalport,0) coordinate (sm);
							\path (e) ++(0,1pt+3pt*\horizontalport) coordinate (em);
							\path (\targethorizontalindex,\verticalindex) ++(-45pt+10pt*\verticalport+2pt*\horizontalport,-45pt+10pt*\horizontalport+2pt*\verticalport) coordinate (m);
							%\path (\targethorizontalindex,\targetverticalindex) ++(-45pt+10pt*\verticalport+2pt*\horizontalport,-10pt+17pt*\verticalindex) coordinate (em);
							\draw[lane,thick] (s) -- (sm) |- (m);
							\draw[lane,thick] (m) |- (em) -- (e);
						}
					}
				}{}
			}
		}
		% %horizontal lines
		% \pgfmathtruncatemacro\lastport{\hamming@horizontal@size - 2}%
		% \foreach \portindex in {0,...,\lastport}
		% {
		% 	\path  (\horizontalindex,\verticalindex) ++(-30pt,-10pt+20pt*\portindex) node[draw] {};
		% 	\pgfmathtruncatemacro{\destination}{\hamming@horizontal@function(\horizontalindex,\portindex,\hamming@horizontal@size)}%
		% 	\ifthenelse{\destination>\horizontalindex}{
		% 		\lanestyle
		% 		%\draw[lane,thick] (\horizontalindex,\verticalindex) ++(-30pt,0) -- ++(2pt+1pt*\portindex,10pt + 2.0pt*\lacin@lane + 10pt*\portindex) -| (\lacin@target,\verticalindex);
		% 		\path (\horizontalindex,\verticalindex) ++(-30pt,-10pt+20pt*\portindex) coordinate (s) ++(0,2pt + 2.0pt*\lacin@lane ) coordinate(sm);
		% 		\path (\lacin@target,\verticalindex) ++(-30pt,-10pt+20pt*\portindex) coordinate (e) ++(0,2pt + 2.0pt*\lacin@lane ) coordinate(em);
		% 		\draw[lane,thick] (s) -- (sm) -- (em) -- (e);
		% 	}{}
		% }
		% %vertical lines
		% \pgfmathtruncatemacro\lastport{\hamming@vertical@size - 2}%
		% \foreach \portindex in {0,...,\lastport}
		% {
		% 	\path  (\horizontalindex,\verticalindex) ++(-10pt+20pt*\portindex,-30pt) node[draw] {};
		% 	\pgfmathtruncatemacro{\destination}{\hamming@vertical@function(\verticalindex,\portindex,\hamming@vertical@size)}%
		% 	\ifthenelse{\destination>\verticalindex}{
		% 		\lanestyle
		% 		%\draw[lane,thick] (\horizontalindex,\verticalindex) ++(0,-30pt) -- ++(10pt + 2.0pt*\lacin@lane + 10pt*\portindex,2pt+1pt*\portindex) |- (\horizontalindex,\lacin@target);
		% 		\path (\horizontalindex,\verticalindex) ++(-10pt+20pt*\portindex,-30pt) coordinate (s) ++(2pt + 2.0pt*\lacin@lane ,0) coordinate (sm);
		% 		\path (\horizontalindex,\lacin@target) ++(-10pt+20pt*\portindex,-30pt) coordinate (e) ++(2pt + 2.0pt*\lacin@lane ,0) coordinate (em);
		% 		\draw[lane,thick] (s) -- (sm) -- (em) -- (e);
		% 	}{}
		% }
	}
}
%\foreach \index in {0,...,\lastindex}
%{
%	\path[draw] (0,-\index) node [anchor=east,shift={(-10pt,0)}] {\index};
%	\draw[very thick] (0,-\index) ++(-10pt,-5pt) rectangle ++(\lastport*40pt+40pt,.5);
%}
}

\newcommand{\rack}[5]{%
\def\rack@sizeI{#1}
\def\rack@sizeV{#2}
\def\rack@sizeX{#3}
\def\rack@sizeY{#4}
\def\rack@function{#5}
\pgfmathtruncatemacro{\vlast}{\rack@sizeV-1}
\pgfmathtruncatemacro{\iports}{\rack@sizeI}
\pgfmathtruncatemacro{\vports}{\rack@sizeV-1}
\pgfmathtruncatemacro{\xports}{\rack@sizeX-1}
\pgfmathtruncatemacro{\yports}{\rack@sizeY-1}
\pgfmathtruncatemacro{\iplast}{\iports-1}
\pgfmathtruncatemacro{\vplast}{\vports-1}
\pgfmathtruncatemacro{\xplast}{\xports-1}
\pgfmathtruncatemacro{\yplast}{\yports-1}
\pgfmathtruncatemacro{\totalports}{\iports+\vports+\xports+\yports}
\pgfmathsetmacro{\pcbmargin}{.1}
\pgfmathsetmacro{\rowpcbheight}{.8}%
\pgfmathsetmacro\pcbwidth{.5}%
\pgfmathsetmacro\pcbheight{\rowpcbheight-2*\pcbmargin}%
\pgfmathsetmacro{\pcbinterval}{\pcbwidth+\pcbmargin}
\pgfmathsetmacro\portinterval{.2}%
\pgfmathsetmacro\portmargin{.1}%
\pgfmathsetmacro\portsize{.1}%
\pgfmathsetmacro\switchwidth{2*\portmargin+\portinterval*\totalports}%
\pgfmathsetmacro{\switchpcbwidth}{\rack@sizeI*(\pcbinterval)+2*\pcbmargin+\switchwidth}%
\pgfmathsetmacro\iportangle{10}%
\pgfmathsetmacro\vportangle{5}%
\pgfmathsetmacro\xportangle{5}%
\pgfmathsetmacro\yportangle{5}%
\foreach \xindex in {0,...,\xplast}
{
	\pgfmathtruncatemacro{\portoffset}{\iports+\vports+\xindex}
	\draw (\rack@sizeI*\pcbinterval+\pcbmargin+\portoffset*\portinterval+\portmargin,\rack@sizeV) coordinate (x bundle port \xindex) circle (3pt);
}
\draw[decoration={brace,raise=4pt},decorate] (x bundle port 0) -- node[anchor=south east,pos=1.00,yshift=4pt]{X bundles} (x bundle port \xplast);
\foreach \yindex in {0,...,\xplast}
{
	\pgfmathtruncatemacro{\portoffset}{\iports+\vports+\xports+\yindex}
	\draw (\rack@sizeI*\pcbinterval+\pcbmargin+\portoffset*\portinterval+\portmargin,\rack@sizeV) coordinate (y bundle port \yindex) circle (3pt);
}
\draw[decoration={brace,raise=4pt},decorate] (y bundle port 0) -- node[anchor=south west,pos=0.00,yshift=4pt]{Y bundles} (y bundle port \yplast);
\foreach \vindex in {0,...,\vlast}
{
	\draw (0,\vindex) rectangle ++(\switchpcbwidth,\rowpcbheight);
	\draw (\rack@sizeI*\pcbinterval+\pcbmargin,\vindex+\pcbmargin) coordinate (switch) rectangle ++(\switchwidth,\pcbheight);
	\foreach \iindex in {0,...,\iplast}
	{
		\draw (\iindex*\pcbinterval,\vindex) ++(\pcbmargin,\pcbmargin) coordinate (server) rectangle ++(\pcbwidth,\pcbheight);
		\draw (switch) ++(\iindex*\portinterval+\portmargin,\portmargin) coordinate (switch port) ++(-.5*\portsize,-.5*\portsize) rectangle ++(\portsize,\portsize);
		\draw (server) ++(\portmargin,\portmargin) coordinate (server port) ++(-.5*\portsize,-.5*\portsize) rectangle ++(\portsize,\portsize);
		\draw (server port) edge[out=\iportangle,in=180-\iportangle] (switch port);
	}
	\foreach \vvindex in {0,...,\vplast}
	{
		\pgfmathtruncatemacro{\portoffset}{\iports+\vvindex}
		\draw (switch) ++(\portoffset*\portinterval+\portmargin,\portmargin) coordinate (switch port) ++(-.5*\portsize,-.5*\portsize) rectangle ++(\portsize,\portsize);
		\pgfmathtruncatemacro{\destination}{\rack@function(\vindex,\vvindex,\rack@sizeV)}%
		\pgfmathtruncatemacro{\cond}{\destination>\vindex && \destination<\rack@sizeV}
		\ifthenelse{\cond=1}{
			\lanestyle
			%\draw[lane,thick] (\horizontalindex,\verticalindex) ++(\portlineoffset,0) -- ++(2pt+1pt*\portindex,1pt + 2.0pt*\lacin@lane + 1pt*\portindex) -| (\lacin@target,\verticalindex);
			%\path (\horizontalindex,\verticalindex) ++(\portlineoffset,\firstportoffset+\verticalportsize*\portindex) coordinate (s) ++(0,2pt + 2.0pt*\lacin@lane ) coordinate(sm);
			%\path (\lacin@target,\verticalindex) ++(\portlineoffset,\firstportoffset+\verticalportsize*\portindex) coordinate (e) ++(0,2pt + 2.0pt*\lacin@lane ) coordinate(em);
			%\draw[lane,thick] (s) -- (sm) -- (em) -- (e);
			%\draw (switch) ++(\portoffset*\portinterval+\portmargin,\portmargin) coordinate (switch port) ++(-.5*\portsize,-.5*\portsize) rectangle ++(\portsize,\portsize);
			\path (\rack@sizeI*\pcbinterval+\pcbmargin,\destination+\pcbmargin) ++(\portoffset*\portinterval+\portmargin,\portmargin) coordinate (destination port);
			\draw[lane,thick] (switch port) edge[out=90-\vportangle,in=-90+\vportangle] (destination port);
		}{}
	}
	\foreach \xindex in {0,...,\xplast}
	{
		\pgfmathtruncatemacro{\portoffset}{\iports+\vports+\xindex}
		\draw (switch) ++(\portoffset*\portinterval+\portmargin,\portmargin) coordinate (switch port) ++(-.5*\portsize,-.5*\portsize) rectangle ++(\portsize,\portsize);
		\draw (switch port) edge[out=90-\xportangle,in=-90+\xportangle] (x bundle port \xindex);
	}
	\foreach \yindex in {0,...,\yplast}
	{
		\pgfmathtruncatemacro{\portoffset}{\iports+\vports+\xports+\yindex}
		\draw (switch) ++(\portoffset*\portinterval+\portmargin,\portmargin) coordinate (switch port) ++(-.5*\portsize,-.5*\portsize) rectangle ++(\portsize,\portsize);
		\draw (switch port) edge[out=90-\yportangle,in=-90+\yportangle] (y bundle port \yindex);
	}
}
}%end rack

%%% Para configuraciones generales que no tengan por qué ser basadas en 1-factorizations.

%%% SWAP
%%% [s,p] -> [p,s+1] si s<p
%%% -> [p-1,s] otherwise
%%% Pero eso es con el puerto en [1,N-1] y yo lo pongo en [0,N-2]. fuck.
\pgfmathdeclarefunction{swap__switch}{3}{%
	\pgfmathtruncatemacro\swap@input@switch{#1}%
	\pgfmathtruncatemacro\swap@input@port{#2}%
	\pgfmathtruncatemacro\swap@size{#3}%
	%\ifthenelse{\swap@input@switch<\swap@input@port}{%
	%	\pgfmathparse{\swap@input@port}%
	%}{%
	%	\pgfmathparse{\swap@input@port-1}%
	%}%
	\pgfmathparse{\swap@input@port+1 - (\swap@input@switch>=\swap@input@port+1)}%
}

\pgfmathdeclarefunction{swap__port}{3}{%
	\pgfmathtruncatemacro\swap@input@switch{#1}%
	\pgfmathtruncatemacro\swap@input@port{#2}%
	%Dammed latex ifthenelse...
	%\ifthenelse{\swap@input@switch<\swap@input@port+1}{%
	%	\pgfmathparse{\swap@input@switch+1}%
	%}{%
	%	\pgfmathparse{\swap@input@switch}%
	%}%
	\pgfmathparse{\swap@input@switch + (\swap@input@switch<\swap@input@port+1) -1}%
}

%%%% CIRCULANT
%%%% [s,p] -> [s+p,n-p]
\pgfmathdeclarefunction{circulant__switch}{3}{%
	\pgfmathtruncatemacro\circulant@input@switch{#1}%
	\pgfmathtruncatemacro\circulant@input@port{#2}%
	\pgfmathtruncatemacro\circulant@size{#3}%
	\pgfmathparse{Mod(\circulant@input@switch+\circulant@input@port+1,\circulant@size)}%
}

\pgfmathdeclarefunction{circulant__port}{3}{%
	\pgfmathtruncatemacro\circulant@input@switch{#1}%
	\pgfmathtruncatemacro\circulant@input@port{#2}%
	\pgfmathtruncatemacro\circulant@size{#3}%
	\pgfmathparse{\circulant@size-\circulant@input@port-2}%
}

\newcommand{\generalcomplete}[2]{%
\def\complete@size{#1}%
\def\complete@function{#2}%
\def\complete@function@switch{\complete@function __switch}%
\def\complete@function@port{\complete@function __port}%
\pgfmathtruncatemacro\lastport{\complete@size - 2}%
\pgfmathtruncatemacro\lastindex{\complete@size - 1}%
\foreach \port in {0,...,\lastport}
{
	\foreach \nextindex in {1,...,\complete@size}
	{
		\pgfmathtruncatemacro{\index}{\nextindex-1}
		%\path[draw] (0,-\index) circle (3pt) node [anchor=east] {\index};
		\path[draw] (\port*40pt,-\index) circle (3pt);
		\pgfmathtruncatemacro{\destination@switch}{\complete@function@switch(\index,\port,\complete@size)}%
		\pgfmathtruncatemacro{\destination@port}{\complete@function@port(\index,\port,\complete@size)}%
		%\pgfmathtruncatemacro{\cond}{\destination@switch>\index && \destination@switch<\complete@size}
		\pgfmathtruncatemacro{\cond}{\destination@switch*\complete@size+\destination@port > \index*\complete@size+\port }
		\ifthenelse{\cond=1}{
			\lanestyle
			\draw[lane,thick,overlay] (\port*40pt,-\complete@size+1+\index) edge [looseness=0.5] (\destination@port*40pt,-\complete@size+1+\destination@switch);
		}{}
	}
}
\foreach \index in {0,...,\lastindex}
{
	%%downwards
	%\path[draw] (0,-\index) node [anchor=east,shift={(-10pt,0)}] (label\index) {Switch \index};
	%%upwards
	\path[draw] (0,-\lastindex+\index) node [anchor=east,shift={(-10pt,0)}, font=\scriptsize] (label\index) {$S =\index$};
	\draw[thin] (0,-\index) ++(-10pt,-5pt) rectangle ++(\lastport*40pt+40pt,.5);
}
}

\makeatother


